On Diffusion-Induced Non-Constant Composition Profiles in the Boundary Layer of Inert Multicomponent Mixtures

In the boundary layer of multicomponent fluid mixtures, the species-specific mass flux in the wall-normal direction is determined by the combination of turbulent-diffusiophoretic diffusion due to composition gradients, and diffusion due to gradients in other scalar fields (e.g. thermophoresis, barophoresis, and forced diffusion). For inert mixtures, a balance must exist between all the diffusive transport mechanisms so that the net diffusive mass flux normal to the wall is zero everywhere. This paper discusses under which conditions non-constant composition profiles are necessary to obtain physico-chemical equilibrium, hence vanishing transport, in the wall-normal direction. Mathematical modeling is employed to demonstrate how this may affect fluid property profiles, wall heat flux, and wall shear stress in an ideal, ternary gas mixture ($H_2 + N_2 + CO_2$) subject to a temperature gradient. It is concluded that competing diffusive transport mechanisms, under certain circumstances, may result in non-constant composition profiles and significantly different wall and bulk compositions, for inert multicomponent mixtures. Hence, wall-normal diffusion in the boundary layer must be accounted for to correctly describe or interpret multicomponent flow systems sensitive to wall friction and heat exchange.

==> Figure1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{013}[cl][cl]{\matlabtextA $CO_2$}%
\psfrag{014}[cl][cl]{\matlabtextA $N_2$}%
\psfrag{015}[cl][cl]{\matlabtextA $H_2$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{016}[tc][tc]{\matlabtextB $y,~\left[\mathrm{m}\right]$}%
\psfrag{017}[bc][bc]{\matlabtextB $x,~\left[\nicefrac{\mathrm{kg}}{\mathrm{kg}}\right]$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10^{-7}$}%
\psfrag{001}[ct][ct]{\matlabtextC $10^{-6}$}%
\psfrag{002}[ct][ct]{\matlabtextC $10^{-5}$}%
\psfrag{003}[ct][ct]{\matlabtextC $10^{-4}$}%
\psfrag{004}[ct][ct]{\matlabtextC $10^{-3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0.0$}%
\psfrag{006}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{007}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.7$}%
%
%% </ytick>

==> Figure2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[cl][cl]{\matlabtextA $\mathrm{With~diffusion}$}%
\psfrag{022}[cl][cl]{\matlabtextA $\mathrm{Without~diffusion}$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{023}[tc][tc]{\matlabtextB $u_{f,\|,bulk},~\left[\nicefrac{\mathrm{m}}{\mathrm{s}}\right]$}%
\psfrag{024}[bc][bc]{\matlabtextB $\rho_{f,wall},~\left[\nicefrac{\mathrm{kg}}{\mathrm{m}^3}\right]$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $1$}%
\psfrag{002}[ct][ct]{\matlabtextC $2$}%
\psfrag{003}[ct][ct]{\matlabtextC $3$}%
\psfrag{004}[ct][ct]{\matlabtextC $4$}%
\psfrag{005}[ct][ct]{\matlabtextC $5$}%
\psfrag{006}[ct][ct]{\matlabtextC $6$}%
\psfrag{007}[ct][ct]{\matlabtextC $7$}%
\psfrag{008}[ct][ct]{\matlabtextC $8$}%
\psfrag{009}[ct][ct]{\matlabtextC $9$}%
\psfrag{010}[ct][ct]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextC $0.15$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.16$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.17$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.18$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.19$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.20$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.21$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.22$}%
\psfrag{019}[rc][rc]{\matlabtextC $0.23$}%
\psfrag{020}[rc][rc]{\matlabtextC $0.24$}%
%
%% </ytick>

==> Figure3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA $\mathrm{With~diffusion}$}%
\psfrag{019}[cl][cl]{\matlabtextA $\mathrm{Without~diffusion}$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{020}[tc][tc]{\matlabtextB $u_{f,\|,bulk},~\left[\nicefrac{\mathrm{m}}{\mathrm{s}}\right]$}%
\psfrag{021}[bc][bc]{\matlabtextB $\rho_{f,wall}\nu_{f,wall},~\left[10^{-8}\mathrm{Pas}\right]$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $1$}%
\psfrag{002}[ct][ct]{\matlabtextC $2$}%
\psfrag{003}[ct][ct]{\matlabtextC $3$}%
\psfrag{004}[ct][ct]{\matlabtextC $4$}%
\psfrag{005}[ct][ct]{\matlabtextC $5$}%
\psfrag{006}[ct][ct]{\matlabtextC $6$}%
\psfrag{007}[ct][ct]{\matlabtextC $7$}%
\psfrag{008}[ct][ct]{\matlabtextC $8$}%
\psfrag{009}[ct][ct]{\matlabtextC $9$}%
\psfrag{010}[ct][ct]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextC $28.9$}%
\psfrag{012}[rc][rc]{\matlabtextC $29.0$}%
\psfrag{013}[rc][rc]{\matlabtextC $29.1$}%
\psfrag{014}[rc][rc]{\matlabtextC $29.2$}%
\psfrag{015}[rc][rc]{\matlabtextC $29.3$}%
\psfrag{016}[rc][rc]{\matlabtextC $29.4$}%
\psfrag{017}[rc][rc]{\matlabtextC $29.5$}%
%
%% </ytick>

==> Figure4.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA $\mathrm{With~diffusion}$}%
\psfrag{019}[cl][cl]{\matlabtextA $\mathrm{Without~diffusion}$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextB $u_{f,\|,bulk},~\left[\nicefrac{\mathrm{m}}{\mathrm{s}}\right]$}%
\psfrag{021}[bc][bc]{\matlabtextB $q_{wall}$, $10^3\nicefrac{\mathrm{W}}{\mathrm{m}^2}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[cb][cb]{\matlabtextC $0$}%
\psfrag{001}[cb][cb]{\matlabtextC $1$}%
\psfrag{002}[cb][cb]{\matlabtextC $2$}%
\psfrag{003}[cb][cb]{\matlabtextC $3$}%
\psfrag{004}[cb][cb]{\matlabtextC $4$}%
\psfrag{005}[cb][cb]{\matlabtextC $5$}%
\psfrag{006}[cb][cb]{\matlabtextC $6$}%
\psfrag{007}[cb][cb]{\matlabtextC $7$}%
\psfrag{008}[cb][cb]{\matlabtextC $8$}%
\psfrag{009}[cb][cb]{\matlabtextC $9$}%
\psfrag{010}[cb][cb]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextC $-16.0$}%
\psfrag{012}[rc][rc]{\matlabtextC $-14.0$}%
\psfrag{013}[rc][rc]{\matlabtextC $-12.0$}%
\psfrag{014}[rc][rc]{\matlabtextC $-10.0$}%
\psfrag{015}[rc][rc]{\matlabtextC $-8.0$}%
\psfrag{016}[rc][rc]{\matlabtextC $-6.0$}%
\psfrag{017}[rc][rc]{\matlabtextC $-4.0$}%
%
%% </ytick>

==> Figure5.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA $\mathrm{With~diffusion}$}%
\psfrag{019}[cl][cl]{\matlabtextA $\mathrm{Without~diffusion}$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{020}[tc][tc]{\matlabtextB $u_{f,\|,bulk},~\left[\nicefrac{\mathrm{m}}{\mathrm{s}}\right]$}%
\psfrag{021}[bc][bc]{\matlabtextB $\tau_{wall},~\left[10^{-3}\mathrm{Pa}\right]$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $1$}%
\psfrag{002}[ct][ct]{\matlabtextC $2$}%
\psfrag{003}[ct][ct]{\matlabtextC $3$}%
\psfrag{004}[ct][ct]{\matlabtextC $4$}%
\psfrag{005}[ct][ct]{\matlabtextC $5$}%
\psfrag{006}[ct][ct]{\matlabtextC $6$}%
\psfrag{007}[ct][ct]{\matlabtextC $7$}%
\psfrag{008}[ct][ct]{\matlabtextC $8$}%
\psfrag{009}[ct][ct]{\matlabtextC $9$}%
\psfrag{010}[ct][ct]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextC $0.0$}%
\psfrag{012}[rc][rc]{\matlabtextC $5.0$}%
\psfrag{013}[rc][rc]{\matlabtextC $10.0$}%
\psfrag{014}[rc][rc]{\matlabtextC $15.0$}%
\psfrag{015}[rc][rc]{\matlabtextC $20.0$}%
\psfrag{016}[rc][rc]{\matlabtextC $25.0$}%
\psfrag{017}[rc][rc]{\matlabtextC $30.0$}%
%
%% </ytick>
